Robust Modeling of Unknown Dynamical Systems via Ensemble Averaged Learning

Recent work has focused on data-driven learning of the evolution of unknown systems via deep neural networks (DNNs), with the goal of conducting long time prediction of the evolution of the unknown system. Training a DNN with low generalization error is a particularly important task in this case as error is accumulated over time. Because of the inherent randomness in DNN training, chiefly in stochastic optimization, there is uncertainty in the resulting prediction, and therefore in the generalization error. Hence, the generalization error can be viewed as a random variable with some probability distribution. Well-trained DNNs, particularly those with many hyperparameters, typically result in probability distributions for generalization error with low bias but high variance. High variance causes variability and unpredictably in the results of a trained DNN. This paper presents a computational technique which decreases the variance of the generalization error, thereby improving the reliability of the DNN model to generalize consistently. In the proposed ensemble averaging method, multiple models are independently trained and model predictions are averaged at each time step. A mathematical foundation for the method is presented, including results regarding the distribution of the local truncation error. In addition, three time-dependent differential equation problems are considered as numerical examples, demonstrating the effectiveness of the method to decrease variance of DNN predictions generally.

==> Integral.tex <==
\subsection{Differential-Integral Equation}

As discussed in Section \ref{sec:others}, the proposed DNN structure can be used to model other
types of equations involving operators such as integrals, see \eqref{integral}. Here, we
consider a differential-integral equation,
\begin{equation}
 \frac{\partial u}{\partial t} + \frac{\partial u}{\partial x} = \frac{1}{2\pi} \int_0^{2\pi} u(y,t) dy - u, {\color{blue} \quad x \in [0,2\pi],}
\end{equation}
with $2\pi$-periodic boundary condition.

The training data are generated on a uniform grid with nodes given by
$x_i = \frac{2\pi}{N}i$, $i = 0,...,N-1$ with $N = 50$. A total number of $10,000$ trajectories with time
step $\Delta t = 5 \times 10^{-4}$ are stored over $n_L=10$ steps \eqref{loss_n}. Note that the training trajectory data are
of very short temporal length, only up to $t=0.005$.  The trajectories are generated by
solving the true equation with the Fourier initial condition \eqref{Fourier} with $a_0=0$, $a_n, b_n \sim U[-1,1]$, and $N_c\sim U\{0,\dots, 10\}$.

%Our DNN structure again has the disassembly block with dimension (width $\times$ depth $\times$ thickness) $51 \times 1 \times 5$, and the assembly layer with dimension (width $\times$ depth $\times$ thickness) $1 \times 1 \times 5$.
The hyperbolic tangent function $\tanh$ is used as the activation
function, along with
cyclic learning with maximum learning rate of $1\times10^{-3}$,
minimum learning rate of $1\times10^{-4}$, and exponential decay rate of
$0.99994$. The DNN model was trained for  
$30,000$ epochs with batch size 50. 

In Fig. \ref{fig:ex3_diff-integ}, the validation results obtained using the initial condition
$$u(x,0) = \exp\left(-\frac{1}{5}\sin(3x)\right) - \frac{1}{2}\cos(x) - 1
$$ are shown. We observe excellent agreement with the reference solution, obtained by solving the true equation.
The results are up to $t=1.5$, which is significantly longer than the temporal length of the training data (for which $t=0.005$). {\color{blue} {We also present prediction tests for 2,000  new initial conditions (20 \% training trajectory number) sampled from the same distribution as in training data. Average $\ell_2$ error and standard deviation is plotted in Fig. \ref{fig:ex3_diff-integ_ErrVsTime}.}}
%%%%%%%%%%
\begin{figure}[htbp]
	\begin{center}
		\includegraphics[width=0.49\textwidth]{Figures/Example3/t=005.eps}
		\includegraphics[width=0.49\textwidth]{Figures/Example3/t=050.eps}
		\includegraphics[width=0.49\textwidth]{Figures/Example3/t=100.eps}
		\includegraphics[width=0.49\textwidth]{Figures/Example3/t=150.eps}
		\caption{Differential-integral
                  equation: Comparison between DNN model prediction and reference solution.}
		\label{fig:ex3_diff-integ}
	\end{center}
\end{figure}

\begin{figure}[htbp]
	\begin{center}
		\includegraphics[width=0.5\textwidth]{Figures/Example3/ErrL2.eps}
		\caption{\color{blue}{Differential-integral
			equation: $\ell_2$ error average over 2,000 new initial conditions. Standard deviation is shaded.}}
		\label{fig:ex3_diff-integ_ErrVsTime}
	\end{center}
\end{figure}
